Step-Back Profiling: Distilling User History for Personalized Scientific Writing

Large language models (LLM) excel at a variety of natural language processing tasks, yet they struggle to generate personalized content for individuals, particularly in real-world scenarios like scientific writing. Addressing this challenge, we introduce STEP-BACK PROFILING to personalize LLMs by distilling user history into concise profiles, including essential traits and preferences of users. To conduct the experiments, we construct a Personalized Scientific Writing (PSW) dataset to study multi-user personalization. PSW requires the models to write scientific papers given specialized author groups with diverse academic backgrounds. As for the results, we demonstrate the effectiveness of capturing user characteristics via STEP-BACK PROFILING for collaborative writing. Moreover, our approach outperforms the baselines by up to 3.6 points on the general personalization benchmark (LaMP), including 7 personalization LLM tasks. Our ablation studies validate the contributions of different components in our method and provide insights into our task definition. Our dataset and code are available at \url{https://github.com/gersteinlab/step-back-profiling}.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}
\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\definecolor{ForestGreen}{rgb}{0.56, 0.93, 0.56}
\definecolor{SkyBlue}{rgb}{0.53, 0.81, 0.92}
\definecolor{Gold}{rgb}{1.0, 0.84, 0.0}
\definecolor{PeachPuff}{rgb}{1.0, 0.85, 0.73}
\definecolor{Goldenrod}{rgb}{0.85, 0.65, 0.13}
\definecolor{LightGrey}{rgb}{0.83, 0.83, 0.83}
\definecolor{Crimson}{rgb}{0.86, 0.08, 0.24}
\definecolor{LightPink}{rgb}{1.0, 0.71, 0.76}

\newcommand{\adjustedcolorbox}[2]{%
  \begingroup
  \setlength{\fboxsep}{0pt}% 
  \colorbox{#1}{\strut #2}%
  \endgroup
}


\newcommand{\greenbox}[1]{\adjustedcolorbox{ForestGreen}{$\displaystyle #1$}}
\newcommand{\bluebox}[1]{\adjustedcolorbox{SkyBlue}{$\displaystyle #1$}}
\newcommand{\yellowbox}[1]{\adjustedcolorbox{Gold}{$\displaystyle #1$}}
\newcommand{\orangebox}[1]{\adjustedcolorbox{PeachPuff}{$\displaystyle #1$}}
\newcommand{\goldbox}[1]{\adjustedcolorbox{Goldenrod}{$\displaystyle #1$}}
\newcommand{\greybox}[1]{\adjustedcolorbox{LightGrey}{$\displaystyle #1$}}
\newcommand{\redbox}[1]{\adjustedcolorbox{Crimson}{$\displaystyle #1$}}
\newcommand{\pinkbox}[1]{\adjustedcolorbox{LightPink}{$\displaystyle #1$}}

\newcommand{\dui}{\textcolor{teal}{\CheckmarkBold}}
\newcommand{\cuo}{\textcolor{purple}{\XSolidBrush}}
\newcommand{\ie}{\emph{i.e.},~}
\newcommand{\eg}{\emph{e.g.},~}
\newcommand{\wrt}{\emph{w.r.t.}~}
\newcommand{\aka}{\emph{aka}~}
% \renewcommand{\paragraph}[1]{\medskip\noindent\textbf{#1.~}}
\newcommand{\todo}{\color{red}{\textbf{TODO.}}~}

\newcommand{\xiaok}[1]{\left(#1\right)}
\newcommand{\zhongk}[1]{\left[#1\right]}
\newcommand{\dak}[1]{\left\{#1\right\}}
\newcommand{\jiaok}[1]{\left<#1\right>}
\newcommand{\shuk}[1]{\left\lVert#1\right\rVert}
\newcommand{\shuks}[1]{\left\lVert#1\right\rVert^2}
\newcommand{\shangk}[1]{\left\lceil #1 \right\rceil}
\newcommand{\xiak}[1]{\left\lfloor #1 \right\rfloor}

\newcommand{\pfrac}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\prob}[2]{p\xiaok{#1 \mid #2}}

\newcommand{\T}{\top}
\newcommand{\dif}{\mathop{}\!\mathrm{d}}
\newcommand{\biset}[1]{\{0,1\}^{#1}}
\newcommand{\ReLU}{\mathrm{ReLU}}
\newcommand{\relu}{\mathrm{ReLU}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\concat}{\mathrm{concat}}
\newcommand{\mean}{\mathrm{mean}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\cov}{\mathrm{cov}}

\newcommand{\range}[1]{{0,1,\cdots,#1}} % 0, 1, ..., N
\newcommand{\Range}[1]{{1,2,\cdots,#1}} % 1, 2, ..., N
\newcommand{\opseq}[3]{{#1_1 #3 #1_2 #3 \cdots #3 #1_{#2}}}
\newcommand{\seq}[2]{\opseq{#1}{#2}{,}}
\newcommand{\xseq}[2]{\opseq{#1}{#2}{\times}}

\newcommand{\bma}{\bm{a}}
\newcommand{\bmb}{\bm{b}}
\newcommand{\bmc}{\bm{c}}
\newcommand{\bmd}{\bm{d}}
\newcommand{\bme}{\bm{e}}
\newcommand{\bmf}{\bm{f}}
\newcommand{\bmg}{\bm{g}}
\newcommand{\bmh}{\bm{h}}
\newcommand{\bmi}{\bm{i}}
\newcommand{\bmj}{\bm{j}}
\newcommand{\bmk}{\bm{k}}
\newcommand{\bml}{\bm{l}}
\newcommand{\bmm}{\bm{m}}
\newcommand{\bmn}{\bm{n}}
\newcommand{\bmo}{\bm{o}}
\newcommand{\bmp}{\bm{p}}
\newcommand{\bmq}{\bm{q}}
\newcommand{\bmr}{\bm{r}}
\newcommand{\bms}{\bm{s}}
\newcommand{\bmt}{\bm{t}}
\newcommand{\bmu}{\bm{u}}
\newcommand{\bmv}{\bm{v}}
\newcommand{\bmw}{\bm{w}}
\newcommand{\bmx}{\bm{x}}
\newcommand{\bmy}{\bm{y}}
\newcommand{\bmz}{\bm{z}}
\newcommand{\bmzero}{\bm{0}}
\newcommand{\bmone}{\bm{1}}
\newcommand{\bmalpha}{\bm{\alpha}}
\newcommand{\bmbeta}{\bm{\beta}}
\newcommand{\bmgamma}{\bm{\gamma}}
\newcommand{\bmdelta}{\bm{\delta}}
\newcommand{\bmepsilon}{\bm{\epsilon}}
\newcommand{\bmtheta}{\bm{\theta}}
\newcommand{\bmiota}{\bm{\iota}}
\newcommand{\bmkappa}{\bm{\kappa}}
\newcommand{\bmlambda}{\bm{\lambda}}
\newcommand{\bmmu}{\bm{\mu}}
\newcommand{\bmnu}{\bm{\nu}}
\newcommand{\bmxi}{\bm{\xi}}
\newcommand{\bmpi}{\bm{\pi}}
\newcommand{\bmrho}{\bm{\rho}}
\newcommand{\bmsigma}{\bm{\sigma}}
\newcommand{\bmtau}{\bm{\tau}}
\newcommand{\bmupsilon}{\bm{\upsilon}}
\newcommand{\bmphi}{\bm{\phi}}
\newcommand{\bmchi}{\bm{\chi}}
\newcommand{\bmpsi}{\bm{\psi}}
\newcommand{\bmomega}{\bm{\omega}}
\newcommand{\bmA}{\bm{A}}
\newcommand{\bmB}{\bm{B}}
\newcommand{\bmC}{\bm{C}}
\newcommand{\bmD}{\bm{D}}
\newcommand{\bmE}{\bm{E}}
\newcommand{\bmF}{\bm{F}}
\newcommand{\bmG}{\bm{G}}
\newcommand{\bmH}{\bm{H}}
\newcommand{\bmI}{\bm{I}}
\newcommand{\bmJ}{\bm{J}}
\newcommand{\bmK}{\bm{K}}
\newcommand{\bmL}{\bm{L}}
\newcommand{\bmM}{\bm{M}}
\newcommand{\bmN}{\bm{N}}
\newcommand{\bmO}{\bm{O}}
\newcommand{\bmP}{\bm{P}}
\newcommand{\bmQ}{\bm{Q}}
\newcommand{\bmR}{\bm{R}}
\newcommand{\bmS}{\bm{S}}
\newcommand{\bmT}{\bm{T}}
\newcommand{\bmU}{\bm{U}}
\newcommand{\bmV}{\bm{V}}
\newcommand{\bmW}{\bm{W}}
\newcommand{\bmX}{\bm{X}}
\newcommand{\bmY}{\bm{Y}}
\newcommand{\bmZ}{\bm{Z}}
\newcommand{\bmGamma}{\bm{\Gamma}}
\newcommand{\bmDelta}{\bm{\Delta}}
\newcommand{\bmTheta}{\bm{\Theta}}
\newcommand{\bmLambda}{\bm{\Lambda}}
\newcommand{\bmXi}{\bm{\Xi}}
\newcommand{\bmPi}{\bm{\Pi}}
\newcommand{\bmSigma}{\bm{\Sigma}}
\newcommand{\bmUpsilon}{\bm{\Upsilon}}
\newcommand{\bmPhi}{\bm{\Phi}}
\newcommand{\bmPsi}{\bm{\Psi}}
\newcommand{\bmOmega}{\bm{\Omega}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbZ}{\mathbb{Z}}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

==> sec/tab-performance.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2.2mm}{
\scalebox{0.75}{
\begin{tabular}{lccccccc}
\toprule
\textsc{Model}
&\textsc{Exact}$\uparrow$  & \textsc{BLEU}$\uparrow$  & \textsc{Levenshtein}$\downarrow$  & \textsc{RDK FTS}$\uparrow$  & \textsc{MACCS FTS}$\uparrow$ & \textsc{Morgan FTS}$\uparrow$ & \textsc{Validity}$\uparrow$ \\

% Forward Prediction
\midrule[1.1pt]
\rowcolor[RGB]{234, 238, 234}
\multicolumn{8}{l}{\textit{Forward Reaction Prediction}} \\
% \color{gray} Chemformer$^*$~\cite{Chemformer} & \color{gray}0.502	&\color{gray}0.834	&\color{gray}6.878	&\color{gray}0.756	&\color{gray}0.821	&\color{gray}0.739	&\color{gray}0.986 \\
\color{gray} Chemformer$^*$~\cite{Chemformer} & \color{gray}0.372 & \color{gray}0.824 & \color{gray}8.097 & \color{gray}0.755 & \color{gray}0.820 & \color{gray}0.717 & \color{gray}0.994 \\
\color{gray} MoleculeTransformers$^*$~\cite{MolecularTransformer} & \color{gray}0.313 & \color{gray}0.663 & \color{gray}11.735 & \color{gray}0.549 & \color{gray}0.619 & \color{gray}0.532 & \color{gray}0.925 \\
Mol-Instruction~\cite{Mol-Instruction} & 0.065 & 0.428 & 24.076 & 0.260 & 0.430 & 0.249 & 0.999 \\
LLama2-7b$^*$~\cite{Llama2} &0.251	&0.658	&13.167	&0.533	&0.630	&0.512	&0.940 \\
Vicuna v1.5-7b$^*$~\cite{Vicuna} &0.250	&0.659	&12.506	&0.513	&0.600	&0.495	&0.903 \\
LlaSMol-Mistral~\cite{LLaSMol} & 0.055	&0.750	&15.558	&0.221	&0.471	&0.202	&0.788 \\
nach0-base~\cite{nach0} &0.331	&0.857	&13.108	&0.628	&0.709	&0.594	&0.977 \\
Text+Chem T5~\cite{Text+ChemT5} &0.236	&0.750	&13.631	&0.523	&0.630	&0.505	&0.967 \\
T5Chem~\cite{T5Chem} &0.313	&0.703	&13.632	&0.535	&0.616	&0.520	&0.965 \\
\midrule
\textbf{\ModelName} & 0.355 & 0.836 & 10.647 &0.646	&0.726	&0.624	&0.973 \\

% Retrosynthesis Prediction
\midrule[1.1pt]
\rowcolor[RGB]{234, 238, 234}
\multicolumn{8}{l}{\textit{Retrosynthesis Prediction}} \\
% \color{gray} Chemformer$^*$ & \color{gray}0.360	&\color{gray}0.791	&\color{gray}14.114	&\color{gray}0.738	&\color{gray}0.826	&\color{gray}0.698	&\color{gray}0.995 \\
\color{gray} Chemformer$^*$ & \color{gray}0.011 & \color{gray}0.611 & \color{gray}21.073 & \color{gray}0.659 & \color{gray}0.730 & \color{gray}0.574 & \color{gray}0.998 \\
\color{gray} Retroformer$^*$ \citep{Retroformer} & \color{gray}0.273 & \color{gray}0.769 & \color{gray}14.768 & \color{gray}0.690 & \color{gray}0.782 & \color{gray}0.647 & \color{gray}0.952 \\
Mol-Instruction & 0.039 & 0.395 & 31.611 & 0.279 & 0.478 & 0.26 & 1.0 \\
LLama2-7b$^*$ &0.220	&0.754	&15.695	&0.649	&0.747	&0.608	&0.933 \\
Vicuna v1.5-7b$^*$&0.220	&0.756	&15.692	&0.658	&0.758	&0.616	&0.943 \\
LlaSMol-Mistral & 0.010	&0.694	&19.719	&0.148	&0.317	&0.119	&0.530 \\
nach0-base &0.173	&0.854	&18.883	&0.574	&0.668	&0.515	&0.892 \\
Text+Chem T5 &0.042 &0.620 &13.952 &0.261 &0.281 &0.206 &0.345 \\
T5Chem &0.208	&0.725	&17.278	&0.595	&0.662	&0.566	&0.994\\
\midrule
\textbf{\ModelName} & 0.275 &0.902 &14.433	&0.655	&0.747	&0.619	&0.980 \\

% Reaction Condition Prediction (Reagent)
\midrule[1.1pt]
\rowcolor[RGB]{234, 238, 234}
\multicolumn{8}{l}{\textit{Reaction Condition Prediction (Reagent)}} \\
LLama2-7b$^*$ &0.312	&0.564	&9.058	&0.560	&0.575	&0.466	&1.0 \\
Vicuna v1.5-7b$^*$ &0.315	&0.585	&8.664	&0.576	&0.587	&0.473	&1.0 \\
nach0-base &0.001	&0.172	&34.212	&0.053	&0.134	&0.039	&0.932\\
Mol-Instruction &0.0	&0.219	&27.108	&0.034	&0.098	&0.030	&1.0\\
T5Chem &0.019	&0.559	&11.044	&0.366	&0.461	&0.374	&0.994\\
\midrule
\textbf{\ModelName} & 0.458	&0.776	&6.206	&0.678	&0.683	&0.601	&0.999\\

% Reaction Condition Prediction (Catalyst)
\midrule[1.1pt]
\rowcolor[RGB]{234, 238, 234}
\multicolumn{8}{l}{\textit{Reaction Condition Prediction (Catalyst)}} \\
LLama2-7b$^*$ &0.680	&0.720	&2.545	&0.882	&0.868	&0.687	&1.0 \\
Vicuna v1.5-7b$^*$ &0.685	&0.703	&2.451	&0.883	&0.869	&0.692	&1.0 \\
nach0-base &0.0	&0.072	&36.442	&0.129	&0.055	&0.009	&0.849 \\
Mol-Instruction &0.0	&0.110	&28.424	&0.031	&0.045	&0.015	&0.999\\
T5Chem &0.022	&0.346	&13.408	&0.146	&0.268	&0.200	&0.996\\
\midrule
\textbf{\ModelName}       & 0.768	&0.814	&1.755	&0.914	&0.895	&0.774	&1.0\\

% Reaction Condition Prediction (Solvent)
\midrule[1.1pt]
\rowcolor[RGB]{234, 238, 234}
\multicolumn{8}{l}{\textit{Reaction Condition Prediction (Solvent)}} \\
LLama2-7b$^*$ &0.311	&0.462	&3.819	&0.452	&0.48	&0.417	&1.0 \\
Vicuna v1.5-7b$^*$ &0.320	&0.436	&3.809	&0.459	&0.486	&0.427	&1.0 \\
nach0-base &0.0	&0.072	&36.442	&0.129	&0.055	&0.009	&0.849\\
Mol-Instruction &0.0	&0.155	&25.117	&0.030	&0.122	&0.035	&1.0\\
T5Chem &0.083	&0.311	&16.224	&0.458	&0.424	&0.397	&0.995\\
\midrule
\textbf{\ModelName}       & 0.419	&0.695	&2.758	&0.529	&0.547	&0.506	&0.912\\

\bottomrule
\end{tabular}
}}
\vskip -0.1in
\caption{\small{
Comparison of various models on forward reaction prediction, retrosynthesis prediction, and reaction condition prediction tasks.  \textcolor{gray}{Model} indicates a domain expert method, and $^*$ denotes our re-implementation. }
}
\label{tab:chemical_reaction}
\end{table*}
% NOTE: we exclude 


\begin{table*}[!htbp]
\centering
\begin{tabular}{@{}c@{\hspace{0.5cm}}c@{}c@{}}
  % first subtable
  \begin{subtable}[t]{0.35\linewidth} % Adjusted width
    \setlength{\tabcolsep}{2.8 pt}
    \renewcommand\arraystretch{1.0}
    \centering
    \scalebox{0.55}{
    \begin{tabular}{lccc}
        \toprule
        \textsc{Method} &\textsc{Reactant} &\textsc{Solvent} &\textsc{Ligand}\\
        \midrule[1.1pt]
        \rowcolor[RGB]{234, 238, 234} \multicolumn{4}{l}{\textit{Reagent Selection}} \\
        \rowcolor[RGB]{255, 255, 255}
        LLama2-7b$^*$& 0.670 & 0.550 & 0.010\\
        Vicuna v1.5-7b$^*$& 0.690 & 0.580 & 0.440\\
        GPT-4$^\dagger$& 0.299 & 0.526 & 0.534 \\
        GAL-30B$^\dagger$~\cite{Galactica}& 0.107 & 0.104 & 0.030 \\
        LLama2-13b-chat$^\dagger$& 0.145 & 0.050 & 0.284 \\
        ChemDFM-13b~\cite{ChemDFM} & 0.240 & 0.120 & 0.350 \\
        \midrule
        \textbf{\ModelName{}}& 0.780 & 0.630 & 0.520 \\
        \bottomrule
    \end{tabular}
    }
  \end{subtable}
  &
  % second subtable
  \begin{subtable}[t]{0.35\linewidth} % Adjusted width
    \setlength{\tabcolsep}{2.8 pt}
    \renewcommand\arraystretch{1.0}
    \centering
    \scalebox{0.55}{
    \begin{tabular}{lccc}
        \toprule
        \textsc{Method} &\textsc{Acc}$\uparrow$ & \textsc{CEN}$\downarrow$ & \textsc{MCC}$\uparrow$ \\
        \midrule[1.1pt]
        \rowcolor[RGB]{234, 238, 234} \multicolumn{4}{l}{\textit{Reaction Type Classification}} \\
        \rowcolor[RGB]{255, 255, 255}
        \color{gray}BERT classifier~\cite{RXNFP} & \color{gray} 0.989 & \color{gray}0.006 & \color{gray}0.989\\
        \color{gray}ContraGIN~\cite{ContraGIN} & \color{gray} 0.993 & \color{gray}0.001 & \color{gray}0.993 \\
        \color{gray}DRFP~\cite{DRFP} & \color{gray} 0.977 & \color{gray}0.011 & \color{gray}0.977\\
        T5Chem & 0.995 & 0.003 & 0.995\\
        LLama2-7b$^*$ & 0.804 & 0.079  & 0.803 \\
        Vicuna v1.5-7b$^*$ & 0.888 & 0.048 & 0.887\\
        \midrule
        \textbf{\ModelName{}} & 0.991 & 0.004 &0.991\\
        \bottomrule
    \end{tabular}
    }
  \end{subtable}
  &
  % third subtable
  \begin{subtable}[t]{0.30\linewidth} % Adjusted width
    \setlength{\tabcolsep}{2.8 pt}
    \renewcommand\arraystretch{1.0}
    \centering
    \scalebox{0.55}{
    \begin{tabular}{lcc}
        \toprule
        \textsc{Method} &\textsc{B-H} &\textsc{S-M} \\
        \midrule[1.1pt]
        \rowcolor[RGB]{234, 238, 234} \multicolumn{3}{l}{\textit{Yield Regression}} \\
        \rowcolor[RGB]{255, 255, 255}
        \color{gray}DFT~\cite{DFT} & \color{gray}0.920 & \color{gray}- \\
        \color{gray}UAGNN~\cite{UAGNN} & \color{gray}0.969 & \color{gray}0.884 \\
        \color{gray}YieldBERT~\cite{YieldBERT} & \color{gray}0.950 & \color{gray}0.815 \\
        T5Chem & 0.970 & - \\
        LLama2-7b$^*$ & -0.476 & 0.121 \\
        Vicuna v1.5-7b$^*$ & -0.131 & 0.151 \\
        \midrule
        \textbf{\ModelName{}} & 0.944 & 0.652 \\
        \bottomrule
    \end{tabular}
    }
  \end{subtable}
\end{tabular}
\vskip -0.1in
\caption{\small{
Comparison with baselines on reagent selection, reaction type classification, and yield regression tasks. $^\dagger$ denotes results from~\cite{ChemDFM}. For reagent selection, we report the result in top-1 accuracy except for \textsc{Ligand Selection} where we report the top 50\% accuracy. For yield task, we report the $R^2$ score.
}}
\label{tab:other}
\vskip -0.2in
\end{table*}
